Assessing Performance Implications of Deep Copy Operations via Microbenchmarking

As scientific frameworks become sophisticated, so do their data structures. Current data structures are no longer simple in design and they have been progressively complicated. The typical trend in designing data structures in scientific applications are basically nested data structures: pointing to a data structure within another one. Managing nested data structures on a modern heterogeneous system requires tremendous effort due to the separate memory space design. In this paper, we will discuss the implications of deep copy on data transfers on current heterogeneous. Then, we will discuss the two options that are currently available to perform the memory copy operations on complex structures and will introduce pointerchain directive that we proposed. Afterwards, we will introduce a set of extensive benchmarks to compare the available approaches. Our goal is to make our proposed benchmarks a basis to examine the efficiency of upcoming approaches that address the challenge of deep copy operations.

==> include/eval_system_table.tex <==

\begin{table}[]
\caption{Our Evaluation Systems}
\label{eval_system_table}
\vspace{-1em}
\footnotesize
% \scriptsize
% \def\arraystretch{0.8}%  1 is the default, change whatever you need
\begin{tabular}{lll}
\hline
                      & Sabine P100          & Sabine V100          \\ \hline
System                & HPE ProLiant XL190r  & HPE Proliant XL270d  \\
CPU                   & Intel Xeon E5-2680v4 & Intel Xeon E5-2680v4 \\
Sockets (Total Cores) & 2 (28)               & 2 (28)               \\
Host RAM              & 256GB                & 256GB                \\
GPU Architecture      & Pascal               & Volta                \\
GPU                   & 2 $\times$ P100      & 8 $\times$ V100      \\
GPU L2 Cache Size     & 4MB                  & 6MB                  \\
GPU Memory            & 16GB                 & 16GB                 \\
PGI Compiler          & 18.4                 & 18.4                 \\
CUDA Toolkit          & 10.0                 & 10.0                 \\ \hline
\end{tabular}
\end{table}



% \begin{table*}[t]
% \caption{Our Evaluation Systems}
% \label{eval_system_table}
% \vspace{-1em}
% \footnotesize
% % \scriptsize
% % \def\arraystretch{0.8}%  1 is the default, change whatever you need
% \begin{tabular}{llll}
% \toprule
%                       & UHPC                 & Sabine P100          & Sabine V100          \\ \midrule
% System                & HPE Apollo XL190r    & HPE ProLiant XL190r  & HPE Proliant XL270d  \\
% CPU                   & Intel Xeon E5-2660v3 & Intel Xeon E5-2680v4 & Intel Xeon E5-2680v4 \\
% Sockets (Total Cores) & 2 (20)               & 2 (28)               & 2 (28)               \\
% Host RAM              & 128GB                & 256GB                & 256GB                \\
% GPU Architecture      & Kepler               & Pascal               & Volta                \\
% GPU                   & 1 $\times$ K80       & 2 $\times$ P100      & 8 $\times$ V100      \\
% GPU Memory            & 8GB                  & 16GB                 & 16GB                 \\
% PGI Compiler          &                      & 18.4                 & 18.4                 \\
% CUDA Toolkit          &                      & 10.0                 & 10.0                 \\ \bottomrule
% \end{tabular}
% \end{table*}



==> include/figure-src-to-src.tex <==
% https://tex.stackexchange.com/questions/139214/how-to-make-a-subfigure-span-the-two-columns-in-ieeetrans-style
% https://tex.stackexchange.com/questions/333249/controlling-subfigure-captions-and-subfigure-placement




% \begin{figure}	
% 	\centering
% 	\begin{subfigure}[!htbp]{0.75\columnwidth}
% 		\centering
% 		\includegraphics[width=1.00\columnwidth]{fig/src-to-src-compiler.pdf}
% % 		\caption{Caption 1}\label{fig:1a}		
% 	\end{subfigure}
%     \quad
% 	\begin{subfigure}[!htbp]{0.75\columnwidth}
% 		\centering
% 		\includegraphics[width=1.00\columnwidth]{fig/src-to-src-compiler.pdf}
% % 		\caption{Caption 1}\label{fig:1a}		
% 	\end{subfigure}
% 	\caption{---}
%     \label{src2src}
% \end{figure}


% \begin{figure*}	
% 	\centering
% 	\begin{subfigure}[t]{0.8\columnwidth}
% 		\centering
% 		\includegraphics{fig/src-to-src-compiler.pdf}
% 		\caption{Caption 1}\label{fig:1a}		
% 	\end{subfigure}
% 	\quad
% 	\begin{subfigure}[t]{0.8\columnwidth}
% 		\centering
% 		\includegraphics{fig/src-to-src-compiler.pdf}
% 		\caption{Caption 2}\label{fig:1b}
% 	\end{subfigure}
% 	\caption{Main figure caption}\label{fig:1}
% \end{figure*}



% \begin{figure*}
%   \centering
%   \begin{minipage}[b]{.4\textwidth}
% 		\centering
% 		\includegraphics[width=1.00\columnwidth]{fig/src-to-src-compiler.pdf}
% 	  \caption{Caption}
% %       \label{label-a}
%   \end{minipage}\qquad
%   \begin{minipage}[b]{.4\textwidth}
% 		\centering
% 		\includegraphics[width=1.00\columnwidth]{fig/src-to-src-compiler.pdf}
% 	  \caption{Caption}
% %       \label{label-b}
%   \end{minipage}
%   \caption{qqq}
%   \label{qqq}
% \end{figure*}








% \begin{figure*}%
%     \centering
%     \begin{subfigure}{.8\columnwidth}
%         \includegraphics[width=\columnwidth]{fig/src-to-src-compiler.pdf}%
%         \caption{cap a}%
%         \label{subfiga}%
%     \end{subfigure}\hfill%
%     \begin{subfigure}{0.9\columnwidth}
%         \includegraphics[width=\columnwidth]{fig/gecko-sample-code.pdf}%
%         \caption{cap b}%
%         \label{subfigb}%
%     \end{subfigure}\hfill%
%     \caption{The proper caption}
%     \label{figabc}
% \end{figure*}

\begin{figure*}%
    \centering
    \includegraphics[width=\textwidth]{fig/gecko-sample-code.pdf}%
    \caption{a) Diagram of \textit{Gecko}'s runtime and source-to-source translator. b) A sample source code annotated with the \textit{Gecko}'s directives. c) A sample of configuration file that resembles the first three sections of the source code (\textit{a}). d) An overview of defined hierarchy in the source code (\textit{b}) and configuration file (\textit{c}).}
    \label{geck-runtime-src-config}
    \vspace{-1em}
\end{figure*}


==> include/hetero-figure.tex <==

\begin{figure}	
	\centering
	\begin{subfigure}[!htbp]{1.05\columnwidth}
		\centering
		\includegraphics[width=1.00\columnwidth]{fig/percentage-speedup.pdf}
	\end{subfigure}
	\caption{Simultaneous execution of benchmark applications on a single core of Intel Xeon (host) and four NVidia GPUs without the \textit{split} placement strategy. The X-axis determines the percentage of iterations executed on the host (for all kernels) and the rest is distributed among GPUs. The Y-axis shows the achieved speedup with respect to 100\% execution on the host. The speedup for the \textit{Host+1GPU} case of \textit{stencil}, \textit{gaussian}, and \textit{lud} is close to 50.}
    \label{percentage-speedup}
    \vspace{-1.5em}
\end{figure}




==> include/introduction.tex <==
Due to advances in semiconductor manufacturing, GPUs~\cite{GPUS_AND_FUTURE_OF_COMPUTING} and MICs (Many Integrated Cores) have been widely adopted in the design of high performance computing (HPC) systems. They provide massively parallel computing capabilities to applications while addressing multicore issues. As an example, NVidia's Volta V100 consumes 35~pJ per floating-point operation at 7,014 GFLOPs, computed as thermal design point (TDP) divided by the peak double-precision floating-point performance, while a modern Intel processor, Xeon E5 2698v3, consumes 385~pJ at 350 GFLOPs. These promising numbers has led to the incorporation of more GPUs into the modern design. Realization of such design is observed in the latest ORNL's supercomputer, Summit, with six NVidia GPUs per node while having only two IBM POWER9 processors. Future exascale computing nodes are expected to embrace such heterogeneity and growth in computational devices \cite{AMM}, which makes utilization of all available resources a non-trivial job. 



==> include/mem_alloc_algo.tex <==


\begin{algorithm}[t]
  \caption{Memory Allocation Algorithm}
  \small  
  \label{mem_alloc_algo}
  \begin{algorithmic}[1]
  	\Require{$gTree$: \textit{Gecko}'s hierarchical tree structure.}
  	\Require{$loc$: the target $Location$.}
    \Ensure{Memory Allocation API.}
    
	\Function{memAlloc}{gTree, loc} 
    
      \State $\algvar{allocFunc} \assign \makeconst{null}$ \Comment{\underline{Chosen Allocation API}}
    
      \If{$\algvar{gTree}.isLeaf(\algvar{loc})$}
        \If{$\algvar{gTree}.getType(\algvar{loc}) == \makeconst{host}$}
          \State $\algvar{allocFunc} \assign malloc$
        \ElsIf{$\algvar{gTree}.getType(\algvar{loc}) == \makeconst{gpu}$}
          \State $\algvar{allocFunc} \assign cudaMalloc$
        \EndIf
      \Else
        \State $\algvar{children} \assign \algvar{gTree}.getChildren()$
        
        \If{$\algvar{children}.areAllMC()$}
          \State $\algvar{allocFunc} \assign malloc$
        \Else
          \State $\algvar{allocFunc} \assign cudaMallocManaged$
        \EndIf
        
      \EndIf

    \EndFunction
  \end{algorithmic}
\end{algorithm}


%         \If{$\algvar{children}.areAllCPU()$}
%           \State $\algvar{allocFunc} \assign malloc$
%         \ElsIf{$\algvar{children}.areAllGPU()$}
%           \State $\algvar{genCriteria} \assign \algvar{children}.prePascal()$
%           \State $\algvar{p2pCriteria} \assign \algvar{children}.p2pAvailable()$
%           \If{$\algvar{genCriteria} \AND \algvar{p2pCriteria}$}
%             \ForEach{$ a, b \in \algvar{children} $}
%               \State $EnableP2P(\algvar{a}, \algvar{b})$  
%             \EndFor
%             \State $\algvar{allocFunc} \assign cudaMalloc$
%           \Else
%             \State $\algvar{allocFunc} \assign cudaMallocManaged$
%           \EndIf
          
%         \Else
%           \State $\algvar{allocFunc} \assign cudaMallocManaged$
%         \EndIf



==> include/min_code_figure.tex <==

\begin{figure}
	\centering
	\begin{subfigure}[!htbp]{1.00\columnwidth}
		\centering
		\includegraphics[width=1.00\columnwidth]{fig/min_code_change.pdf}
% 		\caption{Caption 1}\label{fig:1a}		
	\end{subfigure}
	\caption{Polymorphic capabilities of \textit{Gecko} leads to less source code modifications. We can change the location hierarchy at run time. Our computational target can be chosen at runtime: processors (\textit{b}) or GPUs (\textit{c}). \textit{Gecko} also supports deep hierarchies in order to provide more flexibility to applications (\textit{d}). We are able to extend the hierarchy as workload size changes (\textit{e}).} 
    \label{min_code_change}
%     \vspace{-2em}
\end{figure}



==> include/speedup-figure.tex <==

\begin{figure*}
  \centering
  \begin{minipage}[b]{1.00\textwidth}
		\centering
		\includegraphics[width=1.00\columnwidth]{fig/speedup.pdf}
	  \caption{Speedup of benchmark applications with \textit{Gecko}. a) without split data placement strategy. b) with split data placement strategy. -- \texttt{acc-managed} is OpenACC with UVM and \texttt{acc} is OpenACC without UVM.}
      \label{results-speedup}
  \end{minipage}\qquad
  \begin{minipage}[b]{1.00\textwidth}
		\centering
		\includegraphics[width=1.00\columnwidth]{fig/page-faults.pdf}
	  \caption{Total GPU page faults of benchmark applications with \textit{Gecko}. a) without split data placement strategy. b) with split data placement strategy. -- \texttt{acc-managed} is OpenACC with UVM and \texttt{acc} is OpenACC without UVM.}
      \label{results-gpu-pagefaults}
  \end{minipage}
%   \caption{Speedup results of the benchmark applications.}
%   \label{rodinia-results}
	\vspace{-2em}
\end{figure*}



